Lipschitz Continuous Allocations for Optimization Games

In cooperative game theory, the primary focus is the equitable allocation of payoffs or costs among agents. However, in the practical applications of cooperative games, accurately representing games is challenging. In such cases, using an allocation method sensitive to small perturbations in the game can lead to various problems, including dissatisfaction among agents and the potential for manipulation by agents seeking to maximize their own benefits. Therefore, the allocation method must be robust against game perturbations. In this study, we explore optimization games, in which the value of the characteristic function is provided as the optimal value of an optimization problem. To assess the robustness of the allocation methods, we use the Lipschitz constant, which quantifies the extent of change in the allocation vector in response to a unit perturbation in the weight vector of the underlying problem. Thereafter, we provide an algorithm for the matching game that returns an allocation belonging to the $\left(\frac{1}{2}-\epsilon\right)$-approximate core with Lipschitz constant $O(\epsilon^{-1})$. Additionally, we provide an algorithm for a minimum spanning tree game that returns an allocation belonging to the $4$-approximate core with a constant Lipschitz constant. The Shapley value is a popular allocation that satisfies several desirable properties. Therefore, we investigate the robustness of the Shapley value. We demonstrate that the Lipschitz constant of the Shapley value for the minimum spanning tree is constant, whereas that for the matching game is $\Omega(\log n)$, where $n$ denotes the number of vertices.

==> ja_intro.tex <==
協力ゲームは複数のエージェントが協力することでより大きな利益が得られる場合の意思決定のモデル化である。協力ゲーム理論の主要な関心事項は、grand coalition によって得られる利得を、各エージェントにとって acceptable な方法で allocate することである。協力ゲームのうち、対応するエージェント集合に対する最適化問題によって定義されるようなゲームは \emph{optimization game} と呼ばれている。

それぞれ Matching Game および Minimum Spanning Tree Game によって定式化される、以下の有名な例を考えてみよう。
\begin{itemize}
    \item ダブルスの大会に向けてテニスクラブのメンバーがペアを作る。プレイヤーの各ペアには、その二人が組んだ時の獲得賞金の予測値が定まっている。クラブの全ペアが獲得した賞金をメンバーへと配分するとき、各メンバーにはどれだけの賞金を分配するべきか？
    \item 複数の施設が協力し、発電所からの電気を受けるための送電網を作る。敷設する送電線の各候補にはそれぞれ、敷設のためのコストが定まっている。すべての施設に電気が行きわたるような送電網を構築するとき、各施設はそれぞれどれだけのコストを負担するべきか？
\end{itemize}

これらの例において、ゲームの特性関数はしばしば誤差を含んでいたり、意図的な誤申告によって変化させられたりする。たとえば、以下のようなことが考えられる。
\begin{itemize}
    \item 組んだことのないペアの相性を正確に予測するのは難しい。また、過去に組んで相性の分かっているペアも、その事実を隠すことでより多くの利益が得られるなら、そうするかもしれない。
    \item 自然災害や調査不足による予想外の地形や地盤状況、あるいは地権や景観条例の兼ね合いによって、送電線の敷設にかかるコストは誤って見積もられうる。また各施設は自分の負担を減らす目的で、それらの問題を知りながら隠蔽する、あるいはでっちあげることがあるかもしれない。
\end{itemize}
このような不確かな状況において、ゲームのわずかな perturbation に対して大きく変化する allocation をしてしまうと、以下のような問題が発生しうる。
\begin{itemize}
    \item 獲得賞金額の軽微な見積もりミスによって各プレイヤーの得られる利益が大きく変わってしまうならば、プレイヤーは配分に納得できなくなる。また、だれかが虚偽の申告をして大きく利益を増やしたとしても、虚偽の度合いが小さければ、配分を操作する意図があったことを立証するのが難しくなる。
    \item 電線敷設上の些細な問題の有無が自分の施設の負担額を大幅に増やす可能性を施設は納得できない。また、そうすることで自分の負担額を大幅に減らしたり、競合する施設の負担額を大幅に増やしたりできるのであれば、建設上の小さな問題の多くは隠蔽されるだろうから、リスク管理上の問題が発生する。
\end{itemize}
これらの問題を避けるため、現実の協力ゲームにおいては、ゲームの perturbation の影響を大きく受けないような allocation を用いるのが望ましい。

Before proceeding, 協力ゲーム理論のタームを定義しておこう。The \emph{cooperative game} $(V,\nu)$ はエージェントの集合 $V$ および、エージェントの各部分集合が協力したときに得られる利得を表す \emph{characteristic function} $\nu\colon 2^V \to \mathbb{R}_{\geq 0}$ の組として定義される。\emph{optimization games} とは、$V'\subseteq V$ に対して $\nu(V')$ の値が $V'$ によって定義される最適化問題の最適値で表されるようなゲームである。



コアは最も基本的な解概念であるため、weight vector を受け取って allocation を返すリプシッツ連続なアルゴリズム $\mathcal{A}$ であって、出力がコアに属するものを考えるのは自然なモチベーションである。しかしながら、これができる状況はふたつの理由で限定的である。第一に、ゲームによっては、コアは必ずしも存在するとは限らない。第二に、すべてのインスタンスに対してコアが存在するようなゲームであっても、$\mathcal{A}$ のリプシッツ定数が小さくなるようにコアのベクトルを取ってこられるとは限らない。

==> matching_old.tex <==
\section{Matching Game}
In this section, we prove Theorem~\ref{thm:matching} by giving a Lipschitz continuous algorithm that returns an approximate core allocation of the matching game.
The proof is obtained by constructing an algorithm that satisfies the assumptions of Lemma~\ref{lem:benri_welfare}. Specifically, we prove that an algorithm which returns a vector represented by
\begin{align*}
\int_{b=0}^{1}\Call{MatchingGame}{G,w,b}\mathrm{d}b
\end{align*}
satisfies the assumptions of Lemma~\ref{lem:benri_welfare} for $D=8$ and $L=??$, where the procedure \Call{MatchingGame}{$\cdot$} is given in Algorithm~\ref{alg:matching}.

%Algorithm~\ref{alg:matching} の overview を見ていこう。アルゴリズムはまず、各辺の重み $w_e$ を $2$ べきに比例する量に丸めて修正重み $\widehat{w}_e$ をつくる、ここに比例定数は $b$ に依存する。その後、同じ重みをもつ辺たちを
\snote{write algorithm overview here}
\snote{improve dekita kigasuru. writing}

\begin{algorithm}[t!]
\caption{Lipschitz continuous allocation for the matching game}\label{alg:matching}
\Procedure{\emph{\Call{MatchingGame}{$G,w,b$}}}{
    \KwIn{A graph $G=(V,E)$ where The edge set is indexed with integers in $[1,|E|]$, a weight vector $w \in \mathbb{R}_{\geq 0}^E$, and $b\in [0,1]$.}
    For each $e\in E$ with $w_e>0$, let $w_e\leftarrow 2^{i_e+1+b}$, where $i_e$ be the unique integer such that $2^{i_e+b}\leq w_e < 2^{i_e+1+b}$\;
    $z\leftarrow 0^{V}$\;
    \For{$x\in \mathbb{R}_{\geq 0}$ such that $\{e\in E\colon \widehat{w}_e = x\}\neq \emptyset$}{
        Let $E_x$ be the set of edges in $E$ with $\widehat{w}_e\geq x$\;
        Let $M_x\leftarrow \emptyset$\;
        \For{$e\in E_x$ in ascending order of their indices}{
            \If{None of two endpoints of $e$ are covered by $M_x$}{
                Add $e$ to $M_x$\;
            }
        }
        $z_v\leftarrow \max(z_v,x)$ for all vertices $v\in V$ that are covered by $M_x$\;
    }
    \Return $z$\;
}
\end{algorithm}

\subsection{Core Approximability}

\begin{lemma}
We have
\begin{align*}
    \|\Call{MatchingGame}{G,w,b}\|_1\leq 8\OPT(V,w).
\end{align*}
\end{lemma}
\begin{proof}
Let $x_1 < \dots < x_k$ be the list of non-negative numbers $x$ such that there is an edge with $\widehat{w}_e=x$. Then, any vertex cover of $(G,\widehat{w})$ contains at least $|M_{x_i}|$ vertices of $V$ with weight at least $x_i$. Thus, we have
\begin{align*}
    \VC(V,\widehat{w})\geq \sum_{i=1}^{k}|M_{x_i}|\left(x_i-x_{i-1}\right)\geq \frac{1}{2}\sum_{i=1}^{k}|M_{x_i}|x_i
    \geq \frac{1}{2}\|\Call{MatchingGame}{G,w,b}\|_1,
\end{align*}
where we set $x_0=0$. Furthermore, we have
\begin{align*}
    \VC(V,\widehat{w})\leq 2\VC(V,w)\leq 4\OPT(V,w).
\end{align*}
Combining those inequalities completes the proof.
\end{proof}

\begin{lemma}
Let $V'\subseteq V$. Then, we have
\begin{align*}
    \sum_{v\in V'}z_v\geq \OPT(V',w).
\end{align*}
\end{lemma}
\begin{proof}
Let $e=(u,v)\in E$. Then, we have
\begin{align*}
    w_e\leq \widehat{w}_e\leq \max(z_u,z_v)\leq z_u+z_v,
\end{align*}
where the second inequality is from the fact that at least one of the endpoints of $e$ is covered by $M_{\widehat{w}_e}$ because $M_{\widehat{w}_e}$ is maximal. Let $M$ be the matching that attains $\OPT(V',w)$. Then, we have
\begin{align*}
    \sum_{v\in V'}z_v\geq \sum_{(u,v)\in M}(z_u+z_v)\geq \sum_{e\in M}w_e = \OPT(V',w).
\end{align*}
\end{proof}

\subsection{Lipschitz Contunuity}

Let $f\in E(G)$. We bound
\begin{align*}
    \frac{1}{\delta}\int_{b=0}^{1}\left\|\Call{MatchingGame}{G,w,b} - \Call{MatchingGame}{G,w+\delta \bm{1}_f,b}\right\|_1 \mathrm{d}b,
\end{align*}
which is an upper bound of
\begin{align*}
    \frac{1}{\delta}\left\|\int_{b=0}^{1}\Call{MatchingGame}{G,w,b}\mathrm{d}b - \int_{b=0}^{1}\Call{MatchingGame}{G,w+\delta \bm{1}_f,b}\mathrm{d}b\right\|_1.
\end{align*}
Without loss of generality, we can assume $\delta \leq \min_{e\in E, w_e > 0} w_e$ or $w_f=0$.

When $\widehat{w}_f=\widehat{w}'_f$, \Call{MatchingGame}{$G,w,b$} and \Call{MatchingGame}{$G,w+\delta \bm{1}_f,b$} output the same vector. Otherwise, $E_x\neq E'_x$ happens only when $x=\widehat{w}'_f$ (recall that we assumed $w_f=0$ or $\delta \leq \min_{e\in E, w_e > 0} w_e\leq w_f$). In this case, $M'_x$ may largely differ from $M_x$ for $x=\widehat{w}'_f$. However, the next lemma shows that the set of endpoints of $M_x$ and $M'_x$ are almost the same.

\begin{lemma}\label{lem:diffis2}
Let $X$ and $X'$ be the set of the endpoints of $M_{\widehat{w}'_f}$ and $M'_{\widehat{w}'_f}$, respectively. Then, $|X\triangle X'|\leq 2$.
\end{lemma}
\begin{proof}
Let $H$ be the graph defined by $(X\cup X', M_{\widehat{w}'_f}\cup M'_{\widehat{w}'_f})$. Then, every connected component of $H$ is either a cycle or a path. The vertices contained in $|X\triangle X'|$ are the endpoints of those paths of length at least $2$. Thus, proving that such a path should include $f$ is sufficient.

Let $P$ be a path of length at least two and $e$ be the edge in $P$ with the smallest index. If $e\in M_{\widehat{w}'_f}\setminus M'_{\widehat{w}'_f}$, unless $e=f$, there should be an edge $e'\in M'_{\widehat{w}'_f}\setminus M_{\widehat{w}'_f}$ that shares an endpoint with $e$ and has smaller index than $e$. From the definition of $P$, $e'\in P$. From the definition of $P$, it follows $e'\in P$, but this contradicts the minimality of the index of $e$. The same argument works for the case $e\in M'_{\widehat{w}'_f}\setminus M_{\widehat{w}'_f}$. Therefore, the lemma is proved.
\end{proof}

Lemma~\ref{lem:diffis2} directly implies
\begin{align*}
    \left\|\Call{MatchingGame}{G,w,b} - \Call{MatchingGame}{G,w+\delta \bm{1}_f,b}\right\|_1\leq 2\widehat{w}'_f.
\end{align*}
The following lemma analyzes the probability $\widehat{w}_f\neq \widehat{w}'_f$ happens.
\begin{lemma}
Assume $w'_f\leq 2w_f$. If $b$ is sampled uniformly from $[0,1]$, $\widehat{w}_f\neq \widehat{w}'_f$ happens with probability at most $\frac{\delta}{w_f\log 2}$.
\end{lemma}
\begin{proof}
$\widehat{w}_f\neq \widehat{w}'_f$ happens when there is an integer $i$ with $w_f<2^{i+b}\leq w'_f$, which means $\floor{\log_2 w_f-b}\neq \floor{\log_2 w'_f-b}$. It happens with probability 
\begin{align*}
    \log_2 w'_f - \log_2 w_f = \log_2 \frac{w'_f}{w_f}\leq \frac{1}{\log_2}\cdot \frac{w'_f-w_f}{w_f}=\frac{\delta}{w_f \log 2}.
\end{align*}
\end{proof}

\begin{lemma}
We have
\begin{align*}
    \frac{1}{\delta}\int_{b=0}^{1}\left\|\Call{MatchingGame}{G,w,b} - \Call{MatchingGame}{G,w+\delta \bm{1}_f,b}\right\|_1 \mathrm{d}b\leq \frac{8\delta}{\log 2}.
\end{align*}
\end{lemma}
\begin{proof}
If $w_f=0$, we have
\begin{align*}
    \frac{1}{\delta}\int_{b=0}^{1}\left\|\Call{MatchingGame}{G,w,b} - \Call{MatchingGame}{G,w+\delta \bm{1}_f,b}\right\|_1 \mathrm{d}b
    \leq 2\widehat{w}'_f \leq 4w'_f = 4\delta.
\end{align*}
Otherwise, we have
\begin{align*}
    &\frac{1}{\delta}\int_{b=0}^{1}\left\|\Call{MatchingGame}{G,w,b} - \Call{MatchingGame}{G,w+\delta \bm{1}_f,b}\right\|_1 \mathrm{d}b\\
    &\leq \frac{\delta}{w_f\log 2}\cdot 2\widehat{w}'_f
    = \frac{\delta}{w_f\log 2}\cdot 4w'_f 
    \leq \frac{\delta}{w_f\log 2}\cdot 8w_f\leq \frac{8\delta}{\log 2}.    
\end{align*}
\end{proof}

\subsection{Direct Computation of the Allocation}

==> nisemono.tex <==


\begin{algorithm}[t!]
\caption{Lipschitz continuous imputation for the minimum spanning tree game}\label{alg:mst}
\Procedure{\emph{\Call{VertexCover}{$G,w$}}}{
    \KwIn{A graph $G=(V\cup \{r\},E)$ and a weight vector $w \in \mathbb{R}_{\geq 0}^E$.}
    Sample $\bm{b}$ uniformly from $[0,1]$\;
    For each $e\in E$, let $\bm{l}_e$ be the unique integer such that $2^{\bm{l}_e+\bm{b}}\leq w_e < 2^{\bm{l}_e+1+\bm{b}}$ and $\widehat{\bm{w}}_e\leftarrow 2^{\bm{l}_e}$\;
    $\bm{S}\leftarrow \Call{AuxiliaryTree}{G,\widehat{w}}$ and identify the vertices of $G$ with the corresponding leaves of $\bm{S}$\;
    \For{$e\in E(\bm{S})$ such that $r\not \in \bm{S}_e$}{
        Sample $\bm{x}_e$ uniformly from $[0,\bm{h}_u]$\;
        Let $\mathcal{D}_{e}$ be the set of points $p$ in $\bm{S}_{e}$ with $\bm{h}_p=\bm{x}_e$\;
        Sample $\bm{p}_{e}$ uniformly from $\mathcal{D}_{e}$\;
        Let $\bm{X}_{e}$ be the set of leaves in $T_{\bm{p}_{e}}$\;
        Let $\bm{z}_{e}\leftarrow \frac{h_e}{|\bm{X}_{e}|}\bm{1}_{\bm{X}_{e}}$\;
    }
    \Return $\sum_{e\in E}\bm{z}_{e}$\;
}
\end{algorithm}


Let $e,f$ be two edges of $\bm{S}$. The following lemma bounds $\Pr[\bm{p}_{e}\in f]$.
\begin{lemma}
Let $e$ and $f=(t,t')$ be edges of $S$ such that $r\not \in S_e$. If $f\not \subseteq S_e$, $\Pr[\bm{p}_{e}\in f]=0$. Otherwise, let $k$ be the number of edges on the path between $u$ and $t$ in $S$. Then, we have
\begin{align*}
    \Pr[\bm{p}_{e}\in f]\leq \frac{1}{k+1}\cdot \frac{h_t-h_{t'}}{h_e}.
\end{align*}
\end{lemma}
\begin{proof}
\end{proof}

\begin{lemma}
Let $f=(t,t')$ be an edge of $S$. Then, we have
\begin{align*}
    \sum_{e\in E(S)}\E[\bm{p}_e\in f]\leq (h_t-h_{t'})\cdot O(\log n).
\end{align*}
\end{lemma}
\begin{proof}
\end{proof}

\begin{lemma}
\end{lemma}
\begin{proof}
For $v\in V'$ and $e\in E(S)$ such that $r\not \in S_e$, $\bm{z}_{e,v}>0$ happens only when $e\subseteq \CONN(V')$.
$v\in S_{\bm{p}_e}$, which implies $\bm{p}_e\in \CONN(V')$. Therefore, we have
\begin{align*}
    \sum_{v\in V'}\sum_{e\in E(S)}\E[\bm{z}_{e,v}]
    &= \sum_{e\in E(\CONN(V'))}\E\left[\sum_{v\in S_{\bm{p}_e}\cap V'}\bm{z}_{e,v}\right]
    \leq \sum_{e\in E(S)}\left(h_e\cdot \Pr\left[\bm{p}_e\in \CONN(V')\right]\right)\\
    &= \sum_{e\in E(S)}\int_{x=0}^{h_e}\Pr\left[\bm{p}_e\in \CONN(V')\mid \bm{x}_e=x\right]\mathrm{d}x\\
    &= \sum_{e\in E(S)}\int_{x=0}^{h_e}
\end{align*}
\end{proof}


\begin{itemize}
    \item if $u_{C}$ has no parent, create a vertex $s$ with $h_{s}=\widehat{w}'_f$, add edges $(s,t)$ and $(s,u)$, and delete the edge $(t,u)$.
    \item if $t$ has a parent $s$ with $h_{s}=\widehat{w}'_f$, add an edge $(s,u)$, and delete the edge $(t,u)$. Set $\tau(e)=e$ for all $e\in E(S^b)\setminus \{(t,u)\}$ and $\tau((t,u))=(s,u)$.
    \item if $t$ has a parent $q$ with $h_{q}>\widehat{w}'_f$, create a vertex $s$ with $h_{s}=\widehat{w}'_f$, add edges $(q,s)$, $(s,t)$, and $(s,u)$, and delete edges $(q,t)$ and $(t,u)$. Set $\tau(e)=e$ for all $e\in E(S^b)\setminus \{(q,t),(t,u)\}$, $\tau((q,t))=(q,s)$, and $\tau((t,u))=(s,u)$.
\end{itemize}


$S'^b$ is obtained from $S^b$ by applying the following \emph{rotation} operation:
\paragraph{Rotation}
Let $u$ be the vertex of $S^b$ that corresponds to whichever of the connected components in $\mathcal{C}_{\widehat{w},<\widehat{w}_f}$ that contains one of the endpoints of $f$. Let $t$ be its parent in $S^b$. Then, $S'^b$ is obtained from $S^b$ by replacing the edge $(t,u)$ with an edge from new parent of $u$ to $u$; that is,
\begin{itemize}
    \item if $t$ has no parent, create a vertex $s$ with $h_{s}=\widehat{w}'_f$, add edges $(s,t)$ and $(s,u)$, and delete the edge $(t,u)$. Set $\tau(e)=e$ for all $e\in E(S^b)\setminus \{(t,u)\}$ and $\tau((t,u))=(s,u)$.
    \item if $t$ has a parent $s$ with $h_{s}=\widehat{w}'_f$, add an edge $(s,u)$, and delete the edge $(t,u)$. Set $\tau(e)=e$ for all $e\in E(S^b)\setminus \{(t,u)\}$ and $\tau((t,u))=(s,u)$.
    \item if $t$ has a parent $q$ with $h_{q}>\widehat{w}'_f$, create a vertex $s$ with $h_{s}=\widehat{w}'_f$, add edges $(q,s)$, $(s,t)$, and $(s,u)$, and delete edges $(q,t)$ and $(t,u)$. Set $\tau(e)=e$ for all $e\in E(S^b)\setminus \{(q,t),(t,u)\}$, $\tau((q,t))=(q,s)$, and $\tau((t,u))=(s,u)$.
\end{itemize}
After this operation, if $t$ had exactly two children $u,x$ in $S^b$, $S'^b$ is obtained by contracting vertex $t$ and setting $\tau((s,t))=(s,x)$.


\begin{lemma}
There is at most one $e \in E(S^b)$ such that $\tau(e) = \bot$, and it satisfies $h_e = \widehat{w}_f$. There is at most one $e \in E(S'^b)$ such that $\tau^{-1}(e) = \bot$, and it satisfies $h'_e = \widehat{w}'_f$. Besides these, there is at most one $e \in E(S^b)$ that satisfies $S^b{e}\cap (V\cup {r}) \neq S'^b{\tau(e)}\cap (V\cup {r})$, and it satisfies both $h_e = \widehat{w}_f$ and $h'_e = \widehat{w}'_f$.
\end{lemma}

Let us bound

 We prove the following.
\begin{lemma}
Let $b\in [0,1]$. Then, for all $V'\subseteq V$, we have
\begin{align*}
    \sum_{v\in V'}\sum_{e\in E(S)}\E\left[\bm{z}_{e,v}\mid \bm{b}=b\right]\leq O(\log n)\cdot \OPT(G[V'\cup \{r\}]).
\end{align*}
\end{lemma}
For the remaining part of this section, we fix $b\in [0,1]$ and omit the condition $\bm{b}=b$. Then, $S$, $h$ and $\widehat{w}$ are no longer being random variable.
